Massively Parallel Algorithms for Small Subgraph Counting

Over the last two decades, frameworks for distributed-memory parallel computation, such as MapReduce, Hadoop, Spark and Dryad, have gained significant popularity with the growing prevalence of large network datasets. The Massively Parallel Computation (MPC) model is the de-facto standard for studying graph algorithms in these frameworks theoretically. Subgraph counting is one such fundamental problem in analyzing massive graphs, with the main algorithmic challenges centering on designing methods which are both scalable and accurate. Given a graph $G=(V, E)$ with $n$ vertices, $m$ edges and $T$ triangles, our first result is an algorithm that outputs a $(1+\varepsilon)$-approximation to $T$, with asymptotically \emph{optimal round and total space complexity} provided any $S \geq \max{(\sqrt m, n^2/m)}$ space per machine and assuming $T=\Omega(\sqrt{m/n})$. Our result gives a quadratic improvement on the bound on $T$ over previous works. We also provide a simple extension of our result to counting \emph{any} subgraph of $k$ size for constant $k \geq 1$. Our second result is an $O_{\varepsilon}(\log \log n)$-round algorithm for exactly counting the number of triangles, whose total space usage is parametrized by the \emph{arboricity} $\alpha$ of the input graph. We extend this result to exactly counting $k$-cliques for any constant $k$. Finally, we prove that a recent result of Bera, Pashanasangi and Seshadhri (ITCS 2020) for exactly counting all subgraphs of size at most $5$ can be implemented in the MPC model in total space.

==> 250-overview.tex <==
\section{Overview of Our Techniques}


\subsection{Exact Triangle Counting}
Let $G$ be a graph over $n$ vertices, $m$ edges and arboricity at most $\alpha$. We tackle the task of exactly counting the number of triangles in $G$ using two main ideas. 
Recall that our algorithm works in $O(\log \log n)$ rounds.
In each round $i$, we partition the vertices into low degree vertices $A_i$, and high degree vertices, according to a degree threshold $\gamma_i$, 
 that grows doubly exponentially in the number of rounds.  We then count the number of triangles incident to the set of low degree vertices $A_i$,
 by having each vertex $v\in A_i$, sending its list of active neighbors to all of its active neighbors.
  Any neighbor $u$ of $v$ that detects a common neighbor $w$ to $u$ and $v$, adds the triangle $(u,v,w)$ to the list of discovered triangles. As a triangle might be discovered by more than one vertex, duplicates have to be accounted for. This is done by a careful analysis that tags the triangles according to the degree of their endpoints, and use this information to avoid double counting. Once we add the contribution of the set $A_i$ to the total count of triangles, we  
  remove this set of vertices from the graph, and continue to deal with the new set of low degree vertices in the next iteration. 
  
	Finding common neighbors is also not trivial, as vertices might receive multiple neighbors lists from multiple neighbors in $A_i$, which might exceed the space limit per machine. Hence, each vertex adds to the list of received neighbors list its own list of neighbors, and finding the intersection is done by the list sorting procedure of~\cite{GSZ11}.
  
  
  As each vertex sends its list of neighbors to all of its neighbors, in each iteration $i$, the total memory of messages sent and received is $\sum_{v \in A_i} d{Q_i}(v)^2 \leq |Q_i|\cdot \gamma_i^2$.  Since $G$ has bounded arboricity, and by the setting of the parameter $\gamma_i$, we are promised that in each round the size of the set of remaining vertices $Q_i$ decreases by a factor of $\gamma_i$. 
  Therefore, in the $i^{\textrm{th}}$ iteration, we have that $Q_i =O({n}/{\gamma_i^2})$.
  Therefore, the number of messages sent and received in each iteration is bounded by $|Q_i|\cdot \gamma_i^2=O(n\alpha^2)$. 

%

%
%


\subsection{Approximate Triangle Counting}
Our work reduces approximate triangle counting to exact triangle counting in multiple induced subgraphs of the original graph. Vertex-based partitioning was previously used for triangle counting, e.g., \cite{pagh2012colorful}, but the partitions are disjoint. In our work, obtained partitions might overlap. This allows us to obtain better concentration bounds compared to the prior work, but also brings certain challenges in analysis and MPC implementation.


The high level idea is that each machine $M_i$ samples a subset $V_i$ by including each vertex in $V_i$ with probability $\pV$.
Then each machine computes the induced subgraph $G[V_i]$ and the number of triangles in that subgraph.
The average number of triangles across the machines is an unbiased estimator to the number of triangles in $G$. This approach gives rise to several challenges:
\paragraph{Limited space per machine.}
First, we need to make sure that the induced subgraphs do not exceed the space per machine $O(S)$.  This limit implies a lower bound on our sampling probability, which in turn implies a lower bound on the number of triangles in the graph from which we can guarantee to return a good approximation with high probability. 

\paragraph{Computing the induced subgraph.}
Second, it is unclear how to compute the induced subgraph on each machine without exceeding the total allowed space of $\tilde{O}(m)$.
We tackle this challenge by using a \emph{globally known} hash function $h:V\times [\mM] \rightarrow {0,1}$ to indicate whether vertex $v$ was sampled in machine  vertices into the individual machines. 
By requiring that the  hash function will be known to all machines, we can efficiently compute which edges to send to each subgraph $G[V_i]$. However, in order for all machines to be able to compute the hash function, it has to be of limited space. Hence we cannot hope for a fully independent function, rather we can only use $(S/\log n)$-wise independent  hash function. Still, we manage to show, that we are able to handle the dependencies introduced by the above, even if we allow as little as $O(\log n)$-independence.

\paragraph{High probability bound on the size of the induced subgraphs.} The next challenge is in proving that with high probability, the sizes of the induced subgraphs do not exceed the allowed space per machine. We deal with this by dealing separately with light vertices and heavy vertices. For light vertices it is fairly straightforward to bound their contributed to the number of edges in $G[V_i]$, since their total number of edges is small to begin with. For heavy vertices, we use a variation of Chernoff's inequality that is suitable for bounded dependence variables, and prove that their "sampled" degree behaves as expected. That is, that their number of neighbors in each subgraph where they were sampled behaves as expected.

\paragraph{The number of triangles across the machines concentrates.} Our final challenge is in proving that the sum of triangles over the induced subgraphs is close to its expected value. Here too we have to take into account the dependencies introduced by the hash function.
 
The strategy described above takes advantage  the properties of the MPC model in several ways. First, we use each individual machine to perform a single "experiment" and then view the collection of machines, as repeating this experiment $\mM$ times in parallel. Second, our use of hash functions exploits the unbounded computational power of each machine in order to reduce the round and space complexity at the cost of performing more local computation. 


\subsection{Counting 5-subgraphs and $k$-cliques.}
Our main contribution in this section is a procedure that, given a set of copies of some subgraph $T$, create all copies of all possible extensions of the copies by an additional vertex.  We do so by considering all pairs $(\tau,v)$ where $\tau$ is a copy of $T$, and $v$ is a "neighbor of $\tau$".
We use the arboricity of the graph in order to reduce the space of the above.

We use this procedure both for the task of counting small subgraphs and constant $k$-cliques.


\subsection{Discussion of Our Results}
The MPC model is closely related to the CONGESTED CLIQUE model.
By Theorem 4.3 in~\cite{behnezhad2018semi}, our result for approximate triangle counting (\cref{thm:approximate-counting}) can be implemented in the CONGESTED-CLIQUE model in $O(1)$ rounds. 
This implies an $O(1)$-rounds $(1+\eps)$-approximation algorithm for the number of triangles in a graph in the CONGESTED-CLIQUE, for all graphs for which $T=\Omega(d_{avg})$. 
Furthermore, our results on exact triangle counting(\cref{thm:exact-tri}), can be implemented in $O(1)$ rounds when the arboricity of the graph is bounded by $\alpha=O(n^2/m)$. In particular, the above upper bound on $\alpha$ holds for all graphs for which $m=O(n^{4/3})$. 



